Safety Verification of Unknown Dynamical Systems via Gaussian Process Regression

The deployment of autonomous systems that operate in unstructured environments necessitates algorithms to verify their safety. This can be challenging due to, e.g., black-box components in the control software, or undermodelled dynamics that prevent model-based verification. We present a novel verification framework for an unknown dynamical system from a given set of noisy observations of the dynamics. Using Gaussian processes trained on this data set, the framework abstracts the system as an uncertain Markov process with discrete states defined over the safe set. The transition bounds of the abstraction are derived from the probabilistic error bounds between the regression and underlying system. An existing approach for verifying safety properties over uncertain Markov processes then generates safety guarantees. We demonstrate the versatility of the framework on several examples, including switched and nonlinear systems.

==> sections/problem.tex <==

% problem.tex

We consider a controlled dynamical system
\begin{equation}
    \label{Eqn::Process}
    \begin{split}
        \x(k+1)=f( \x(k,u_k)), \quad  &\x(k) \in  \mathbb{R}^n, \u(k) \in \mathcal{U},\\
        \observation_k=\x_{k}+ \mathbf{\epsilon}_k(u_k), \quad  & \observation_k \in \mathbb{R}^n, \\
        \mathbf{\epsilon}_k(u_k)\sim \mathcal{N}(0,\sigma^2(u_k)\cdot {I}_n)
    \end{split}
\end{equation}
where $f$ is a possibly non-linear and unknown function that represents the dynamics of the underlying system, which we assume to be Lipschitz continuous, $\mathcal{U}$ is a finite set of actions, and $\mathbf{\epsilon}$ is a noise term, which we assume to be independent Gaussian with zero mean and diagonal covariance matrix $\sigma^2(u)\cdot I_n$ for each $u \in \mathcal{U}$ with $I_n$ being the identity matrix of dimension $n$. If $f$ were completely unknown, this may lead to an ill-posed problem. Therefore, in this paper we make the following assumption, which guarantees that $f$ can be learned via GP regression.
\begin{assumption}
\label{assump:smoothnes}
Let $k:\mathbb{R}^n\times \mathbb{R}^n\to \mathbb{R}_{> 0}$ be a given kernel, which is Lipschitz continuous. Then, for each $u\in \mathcal{U}$  and $i\in \{1,...,n \},$ $ f_i(\cdot,u)$,the $i-th $ component of $f(\cdot,u),$ is a sample from a Gaussian process with zero mean and covariance given by the kernel $k$. 
\end{assumption}
\noindent
Assumption \ref{assump:smoothnes} limits the class of functions that we can consider in Process \ref{Eqn::Process}. In fact, if we let $\phi_1,...,\phi_{\infty}$ be the Mercer's decomposition  of kernel $k$ \cite{mercer1909xvi} and call $\mathcal{F}=\{ g\, : \,\exists \lambda_i,i=1,...,\infty, \, \text{s.t. } g=\sum_{i=1}^{\infty} \lambda_i \phi_i  \}$, then Assumption \ref{assump:smoothnes} implies  $f_i(\cdot,u) \in \mathcal{F}$, i.e, each component of $f(\cdot,u)$ is in $\mathcal{F}$.
In the case of a universal kernel, such as the widely-used squared exponential kernel, this assumption is equivalent to $f \in \mathcal{F}$, where $\mathcal{F}$ is a dense set of $\mathcal{C}(X)$, the set of continuous functions in $X$, for any compact set $X\subset \mathbb{R}^n$ \cite{steinwart2001influence}. 
%\LL{This is the underlying assumption you make when you use GP regression. Then, for each of the bounds in the various paper we can make the specific additional assumptions directly in their statement.}

Let $\omega(k)=y_0 \xrightarrow{u_0} y_1 \xrightarrow{u_1}  \ldots \xrightarrow{u_{k-1}} y_k,$ $y_0,..,y_k\in \mathbb{R}^n$ be a trajectory of Process \ref{Eqn::Process} up to time $k$. Then, a strategy $\pi(\omega(k))\in  \mathcal{U}$ is a measurable function that selects the action at time $k$ given the trajectory of the system up to that time.
 In this paper, we consider the following problem, which seeks to compute the probability that the initial states of $\x$ are safe for a given time horizon for all possible strategies.
 \begin{problem}
 \label{ProbForm}
 Let $\mathcal{D}=((x_i,y_i,u_i)| i\in \{1,...,n_{\mathcal{D}} \})$ be $n_{\mathcal{D}}$ samples from Process \eqref{Eqn::Process}.  Then, for a safe set $\SafeSet\subset \mathbb{R}^n$, a time-horizon $[0,T]\subseteq \mathbb{N}$, and $x\in\SafeSet$ compute
 \begin{align*}
     &p_{\min}(x) = \\
     &\quad \min_{\pi} \Pr(\forall k \in [0,T], \x(k)\in\SafeSet | \x(0)=x,\pi,\mathcal{D}),\\
    & p_{\max}(x) =\\
    &\quad \max_{\pi} \Pr(\forall k \in [0,T], \x(k)\in\SafeSet | \x(0)=x,\pi,\mathcal{D}).
 \end{align*}
 That is, $[p_{\min}(x),p_{\max}(x)]$ represents the ranges of safety probabilities for all possible strategies starting from state $x$.
 \end{problem}
 \noindent
% \LL{This really depends on the assumptions. If $f$ is sampled from a GP, then we have that Pr is Gaussian. If we use RKHS, then $Pr$ is just generated from the noise.}
Note that Problem \ref{ProbForm} is probabilistic. This is necessary because of our partial knowledge of $\x$. % and our assumption that $f$ is sampled from a GP with a given kernel $k$ (Assumption \ref{assump:smoothnes}). 
In particular, $\Pr$ is the probability measure induced by the assumption that $f$ has a Gaussian prior distribution (Assumption \ref{assump:smoothnes}) and that the observation noise  $\epsilon$ is also Gaussian \cite{rasmussen2003gaussian}.
Note also that in Problem \ref{ProbForm} we do not require one to compute the strategy $\pi$ that maximizes (or minimize) the safety probability; we are just interested in checking if a given safety probability threshold is guaranteed for all possible strategies.



\subsection{Approach}

Our approach to solve Problem \ref{ProbForm} is through abstractions in terms of {\imdp}s. A crucial part of the abstraction process is the derivation of upper and lower bounds for the transition probability of $\x_k$ to  $q_j \subset \mathbb{R}^n$ given that $\mathbf{x}_{k-1}\in q_i \subset \mathbb{R}^n$. In Section \ref{sec:abstraction}, we show how these bounds can be computed using GP regression by formally taking into account the uncertainty in the learning process. Finally, in Section \ref{sec:verification}, we show that our resulting method is guaranteed to compute upper and lower bounds of $p_{min}(x)$ and $p_{max}(x)$ for all $x\in \SafeSet$. First, in Section \ref{sec:prelim}, we introduce background on Gaussian process regression and discrete Markov models.
\LL{Mention that we can extend to NIPS bounds}
